Ridge from jet-medium interaction in p-Pb collisions at $\sqrt{s_{NN} }$ = 5.02 TeV

In this paper we report the effect of the jet-medium interplay as implemented in EPOS 3 on the ridge like structure observed in high multiplicity p-Pb collisions at $\sqrt{s_{NN}} = $ 5.02 TeV. EPOS 3 takes into account hydrodynamically expanding bulk matter, jets and the jet-medium interaction. The basis of this model is multiple scatterings where each scattering finally produces flux tube / string. In the higher multiplicity event classes where the flux tube/string density is higher, there is a finite probability that the strings will pick up quarks and antiquarks (or diquarks) from the bulk (core) for flux tube breaking to produce jet hadrons (corona) instead of producing them via usual Schwinger mechanism. This will eventually create a correlation between core and corona and also influence the corona-corona correlation as the corona particles containing quarks and antiquarks (or diquarks) from the bulk also carry the fluid information. We report the relative contributions of the core-core, core-corona, corona-core and corona-corona correlations towards the ridge in the high and low multiplicity p-Pb collisions at $\sqrt{s_{NN}} = $ 5.02 TeV using the data generated by EPOS 3. The multiplicity evolution of the ridges in all the cases is also reported.

==> dlnote <==

TITLE:         Ridge from jet-medium interaction in $p$-Pb collisions at $\sqrt{s_{NN}} = 5.02$ TeV
AUTHORS:       Sarkar,Debojit / Chattopadhyay,Subhasis
FIRST AUTHOR:  Sarkar,Debojit
CODE NUMBER:   CV10471
APS CONTACT:   Christopher Wesselborg

INSTRUCTIONS TO PRODUCTION DEPARTMENT:

No pre-marked manuscript

General:
    

Figures:
    

Memos:
    

INSTRUCTIONS TO AUTHOR:
    

REFERENCES CHECKED AGAINST EDITORIAL DATABASE:

REFERENCE ERRORS: Mon Mar 20 09:45:03 EDT 2017


[8a] {epos_massordering_flow_pPb} K. Werner et al., Phys.Rev.Lett. 112, 23 (2014)
Translated as: [prl] Physical Review Letters 112, 23 (2014)
MS: WernerETAL,K./
DB: 
Submitted to journal -- possible matches:
No matches found for author (WernerETAL,K)

[9] {epos_ridgein_pp} K. Werner, Iu. Karpenko, T. Pierog., Phys.Rev.Lett. 106, 122004 (2011)
Translated as: [prl] Physical Review Letters 106, 122004 (2011)
MS: Werner,K./Karpenko,I./T.Pierog./
DB: Werner,K./Karpenko,I./Pierog,T./
WARNING: name mismatch

[13a] {epos_radialflow_spectra_pPb} K. Werner et al., Phys.Rev. C 89, 6 (2014)
Translated as: [prc] Physical Review C 89, 6 (2014)
MS: WernerETAL,K./
DB: 
Submitted to journal -- possible matches:
No matches found for author (WernerETAL,K)

[14] {epos_model_descrip} K. Werner et al., Phys.Rev. C 82, 044904 (2010)
Translated as: [prc] Physical Review C 82, 044904 (2010)
MS: WernerETAL,K./
DB: Werner,K./Karpenko,I./Pierog,T./Bleicher,M./Mikhailov,K./
WARNING: use of et al. discouraged for references with only a few authors
WARNING: first-author name mismatch
No database matches found for author (WernerETAL,K)

Found 4 errors in 20 references (10 checkable)


EPRINT HITS: Mon Mar 20 09:45:03 EDT 2017

None


==> starter <==
%ACC CV10471
%NM Sarkar
%PAGES 6
%FIGS 5
%
%REM Corresponding author
%ADDR1 Dr. Debojit Sarkar
%
%REM Communications data:
%EMAIL:  debojit03564@gmail.com
%
%DL 20Mar2017
%JN C
%SC C-19G
%LH DEBOJIT SARKAR AND SUBHASIS CHATTOPADHYAY
%TT RIDGE FROM JET-MEDIUM INTERACTION IN $p$-Pb ...
%CP  CPY
%CPTXT American Physical Society
%CPHOLDER American Physical Society
%CPURL http://www.aps.org/
%TL Ridge from jet-medium interaction in $p$-Pb collisions at $\sqrt{s_{NN}}
%TL = 5.02$ TeV
%AU <fname>Debojit</fname><surname>Sarkar</surname>
%AU <fname>Subhasis</fname><surname>Chattopadhyay</surname>
%AI
%RD 21 August 2016
%RDREV 1 March 2017
%FL ETEX-Y EFIG-C PDF-Y
%TYPE: REGULAR ARTICLE
%
%END DATA

